Factoring Polynomials over Finite Fields with Linear Galois Groups: An Additive Combinatorics Approach

Let $\tilde{f}(X)\in\mathbb{Z}[X]$ be a degree-$n$ polynomial such that $f(X):=\tilde{f}(X)\bmod p$ factorizes into $n$ distinct linear factors over $\mathbb{F}_p$. We study the problem of deterministically factoring $f(X)$ over $\mathbb{F}_p$ given $\tilde{f}(X)$. Under the generalized Riemann hypothesis (GRH), we give an improved deterministic algorithm that computes the complete factorization of $f(X)$ in the case that the Galois group of $\tilde{f}(X)$ is (permutation isomorphic to) a linear group $G\leq \mathrm{GL}(V)$ on the set $S$ of roots of $\tilde{f}(X)$, where $V$ is a finite-dimensional vector space over a finite field $\mathbb{F}$ and $S$ is identified with a subset of $V$. In particular, when $|S|=|V|^{\Omega(1)}$, the algorithm runs in time polynomial in $n^{\log n/(\log\log\log\log n)^{1/3}}$ and the size of the input, improving Evdokimov's algorithm. Our result also applies to a general Galois group $G$ when combined with a recent algorithm of the author. To prove our main result, we introduce a family of objects called linear $m$-schemes and reduce the problem of factoring $f(X)$ to a combinatorial problem about these objects. We then apply techniques from additive combinatorics to obtain an improved bound. Our techniques may be of independent interest.

==> preamble.tex <==
\usepackage{amsfonts,amssymb,amsmath,amsthm}
\usepackage{mathtools}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{newtxtext}
\usepackage{hhline}
\usepackage{makecell}
\renewcommand\theadalign{bc}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}
\usepackage{stackengine}
\usepackage{tikz-cd}
\usepackage[hidelinks]{hyperref}
\usepackage[shortlabels]{enumitem}

\emergencystretch=1em

%\DeclareUnicodeCharacter{012D}{\u{\i}}
 
   
%\OnehalfSpacing*

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
%\newtheorem{prob}{Problem}[section]
%\newtheorem*{prob*}{Problem}
%\newtheorem{cond}{Condition}[section]
\newtheorem{assumption}{Assumption}
\newtheorem*{question*}{Question}
\newtheorem*{acknowledgment}{Acknowledgments}
 
\theoremstyle{remark}
\newtheorem*{remark*}{Remark}
 

\newcommand{\nospacepunct}[1]{\makebox[0pt][l]{\,#1}}

\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\aut}{\mathrm{Aut}}
\newcommand{\sym}{\mathrm{Sym}}
\newcommand{\alt}{\mathrm{Alt}}
\newcommand{\gal}{\mathrm{Gal}}
\renewcommand{\hom}{\mathrm{Hom}}
\newcommand{\h}{\mathrm{H}}
\newcommand{\map}{\mathrm{Map}}
\renewcommand{\ker}{\mathrm{ker}}
\newcommand{\im}{\mathrm{Im}}
\newcommand{\twr}{\operatorname{twr}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\cha}{\mathrm{char}}
\newcommand{\rad}{\mathrm{Rad}}
\newcommand{\p}{\mathfrak{p}}
\newcommand{\gl}{\mathrm{GL}}
\newcommand{\gammal}{\mathrm{\Gamma L}}
\newcommand{\pgl}{\mathrm{PGL}}
\newcommand{\pgammal}{\mathrm{P\Gamma L}}
\newcommand{\agl}{\mathrm{AGL}}
\newcommand{\proj}{\mathbb{P}}
\newcommand{\soc}{\mathrm{soc}}
\newcommand{\inn}{\mathrm{Inn}}
\newcommand{\out}{\mathrm{Out}}
\newcommand{\hol}{\mathrm{Hol}}
\newcommand{\cl}{\mathrm{Cl}}
\newcommand{\lin}{\mathrm{Lin}}
\DeclareMathOperator{\codim}{codim}
